A Gaze into the Internal Logic of Graph Neural Networks, with Logic

Graph Neural Networks share with Logic Programming several key relational inference mechanisms. The datasets on which they are trained and evaluated can be seen as database facts containing ground terms. This makes possible modeling their inference mechanisms with equivalent logic programs, to better understand not just how they propagate information between the entities involved in the machine learning process but also to infer limits on what can be learned from a given dataset and how well that might generalize to unseen test data. This leads us to the key idea of this paper: modeling with the help of a logic program the information flows involved in learning to infer from the link structure of a graph and the information content of its nodes properties of new nodes, given their known connections to nodes with possibly similar properties. The problem is known as graph node property prediction and our approach will consist in emulating with help of a Prolog program the key information propagation steps of a Graph Neural Network's training and inference stages. We test our a approach on the ogbn-arxiv node property inference benchmark. To infer class labels for nodes representing papers in a citation network, we distill the dependency trees of the text associated to each node into directed acyclic graphs that we encode as ground Prolog terms. Together with the set of their references to other papers, they become facts in a database on which we reason with help of a Prolog program that mimics the information propagation in graph neural networks predicting node properties. In the process, we invent ground term similarity relations that help infer labels in the test set by propagating node properties from similar nodes in the training set and we evaluate their effectiveness in comparison with that of the graph's link structure. Finally, we implement explanation generators that unveil performance upper bounds inherent to the dataset. As a practical outcome, we obtain a logic program, that, when seen as machine learning algorithm, performs close to the state of the art on the node property prediction benchmark.

==> eptcsdata.tex <==
\providecommand{\firstpage}{93}
\providecommand{\publicationstatus}{Y. Lierler, J.F. Morales, C. Dodaro, V. Dahl, M. Gebser, T. Tekle (Eds.):\\ International Conference on Logic Programming 2022 (ICLP'22).\\
EPTCS 364, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.364.9}{10.4204/EPTCS.364.9}}
\pdfoutput=1


==> pheader19.tex <==
\usepackage{graphicx}
\usepackage{mathptmx}
\usepackage{tikz-qtree}
\usepackage{filecontents}
\usepackage{csvsimple}
\usepackage{amsfonts,amsmath}
%\usepackage{subfig} % creates problems - fails maketitile
\usepackage{url}
\usepackage{verbatim}
\usepackage{color}
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

\definecolor{lgray}{gray}{0.95}
\definecolor{lblue}{rgb}{0.90,0.90,1.00}
\definecolor{lyellow}{rgb}{1.00,1.00,0.70}

\usepackage{listings}
\lstloadlanguages{Prolog}
% parameters in this will be overriden by same for {code}
% so this will look the same - except that it will not be treated as code

%\newtheorem{prop}{Proposition}
%\newtheorem{conj}{Conjecture}
%\newtheorem{fact}{Fact}
%\newtheorem{df}{Definition}
%\newtheorem{lem}{Lemma}
\newtheorem{ex}{Example}
%\newtheorem{theo}{Theorem}

\newenvironment{codex}{\small\verbatim}{\endverbatim\normalsize}

\newcommand{\colorON}{\lstset{backgroundcolor=\color{lyellow}}}
\newcommand{\colorOFF}{\lstset{backgroundcolor=\color{white}}}


\let\codeh\comment 

\lstnewenvironment{code}
    {\lstset{}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    \lstset{
      basicstyle=\small\ttfamily,
      % frame=single, 
      backgroundcolor=\color{lgray},
      flexiblecolumns=false,
      basewidth={0.5em,0.45em},        
    }

\newcommand{\BI}[0]{\begin{itemize}}
\newcommand{\EI}[0]{\end{itemize}}
\newcommand{\I}[0]{\item}
\newcommand{\BE}[0]{\begin{enumerate}}
\newcommand{\EE}[0]{\end{enumerate}}
\newcommand{\PP}[0]{ \vskip 0.6cm }
\newcommand{\BX}[0]{\begin{ex}}
\newcommand{\EX}[0]{\end{ex}}
\newcommand{\BV}[0]{\begin{verbatim}}
\newcommand{\EV}[0]{\end{verbatim}}

\newcommand{\BF}[0]{\begin{filecontents*}{data.csv}}
%\newcommand{\EF}[0]{\end{filecontents*}} NOT WORKING
  
\newcommand{\BQ}[0]{\color{blue}\begin{quote}}
\newcommand{\EQ}[0]{\end{quote}\color{black}}  
  
  
% \PIC{1 xlabel}{2 ylabel}{3 Title Label}{4 label}{
\newcommand{\PIC}[4]{
\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}
\begin{axis}[xlabel={#1},ylabel={#2}]
\addplot table [col sep=comma] {data.csv};
\end{axis}
\end{tikzpicture}
\end{center}
\caption{#3}
\label{#4}
\end{figure}
}  

  
% \LPIC{1 xlabel}{2 ylabel}{3 Title Label}{4 label}{
\newcommand{\LPIC}[4]{%\small
\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}
\begin{semilogyaxis}[xlabel={#1},ylabel={#2} (log. scale)]
\addplot table [col sep=comma] {data.csv};
\end{semilogyaxis}
\end{tikzpicture}
\end{center}
\caption{#3}
\label{#4}
\end{figure}
}  

% \PICS{1 xlabel}{2 ylabel}{3 legend1}{5 legend2}{5 Title Label}{6 label}{
\newcommand{\PICS}[6]{%\small
\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}
\begin{axis}[xlabel={#1},ylabel={#2},
		legend entries={#3,#4},
		legend style={
%			at={(1.03,0.5)},
      at={(0.50,1.03)},
			anchor=south
		}
]
\addplot table [x=a,y=b,col sep=comma] {data.csv};
\addplot table [x=a,y=c,col sep=comma] {data.csv};
\end{axis}
\end{tikzpicture}
\end{center}
\caption{#5}
\label{#6}
\end{figure}
}  

% \LPICS{1 xlabel}{2 ylabel}{3 legend1}{5 legend2}{5 Title Label}{6 label}{
\newcommand{\LPICS}[6]{%\small
\begin{figure}[htbp]
\begin{center}
\begin{tikzpicture}
\begin{semilogyaxis}[xlabel={#1},ylabel={#2} (log. scale),
		legend entries={#3,#4},
		legend style={
%			at={(1.03,0.5)},
      at={(0.50,1.03)},
			anchor=south
		}
]
\addplot table [x=a,y=b,col sep=comma] {data.csv};
\addplot table [x=a,y=c,col sep=comma] {data.csv};
\end{semilogyaxis}
\end{tikzpicture}
\end{center}
\caption{#5}
\label{#6}
\end{figure}
}  
   
    
\def \bscale1 {0.25}
\def \bscale {0.25}
\def \N {\mathbb{N}}
\def \T {\mathbb{T}}

% \FIG{Label}{Title}[scale]{file.suf}
\newcommand{\FIG}[4]{
\begin{figure}[htbp]
\centering
{\includegraphics[scale=#3]{../figs/#4}}
\caption{#2}
\label{#1}
\end{figure}
}

% \DFIG{Label}{Title}[scale]{file.suf}
\newcommand{\DFIG}[4]{
\begin{figure*}[htbp]
\centering
{\includegraphics[scale=#3]{../figs/#4}}
\caption{#2}
\label{#1}
\end{figure*}
}


% \FIG{Label}{Title}[scale]{file.suf}
\newcommand{\CFIG}[4]{
\begin{figure}[htbp]
\centering
{\includegraphics[scale=#3,viewport=100 100 500 500,clip]{../figs/#4}}
\caption{#2}
\label{#1}
\end{figure}
}
% totalheight=0.4\textheight


% \HFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\HFIGS}[6]{
\begin{figure}[htbp]
  \centering
  \subfloat[#3]{
    {\includegraphics[scale=0.60]{../figs/#5}}}   
  \subfloat[#4]{
    {\includegraphics[scale=0.60]{../figs/#6}}}
  \caption{#2}
  \label{#1}
\end{figure}
}

% \VFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}
\newcommand{\VFIGS}[6]{
\begin{figure}[htbp]
  \begin{center}
    {\includegraphics[scale=0.40]{../figs/#5}}
    {\includegraphics[scale=0.40]{../figs/#6}}
  \caption{#2: {\em #3} and {\em #4}}
  \label{#1}
  \end{center}
\end{figure}
}


% \VSFIGS{Label}{Title}{Title1}{Title2}{PNG1}{PNG2}{Scale}
\newcommand{\VSFIGS}[7]{
\begin{figure}[htbp]
  \begin{center}
    {\includegraphics[scale=#7]{../figs/#5}}
    {\includegraphics[scale=#7]{../figs/#6}}
  \caption{#2 #3 #4}
  \label{#1}
  \end{center}
\end{figure}
}

% CSV{Title}{Label}
\newcommand{\CSV}[2]{
\begin{figure}[htbp]
\begin{center}
\csvautotabular{data.csv}
\caption{#1}
\label{#2}
\end{center}
\end{figure}
}




==> prolog.tex <==
%\usepackage[top=1in]{geometry}
\usepackage{listings}
\usepackage{xcolor}

% --- ugly internals for language definition ---
%
\makeatletter

% initialisation of user macros
\newcommand\PrologPredicateStyle{}
\newcommand\PrologVarStyle{}
\newcommand\PrologAnonymVarStyle{}
\newcommand\PrologAtomStyle{}
\newcommand\PrologOtherStyle{}
\newcommand\PrologCommentStyle{}

% useful switches (to keep track of context)
\newif\ifpredicate@prolog@
\newif\ifwithinparens@prolog@

% save definition of underscore for test
\lst@SaveOutputDef{`_}\underscore@prolog

% local variables
\newcount\currentchar@prolog

\newcommand\@testChar@prolog%
{%
  % if we're in processing mode...
  \ifnum\lst@mode=\lst@Pmode%
    \detectTypeAndHighlight@prolog%
  \else
    % ... or within parentheses
    \ifwithinparens@prolog@%
      \detectTypeAndHighlight@prolog%
    \fi
  \fi
  % Some housekeeping...
  \global\predicate@prolog@false%
}

% helper macros
\newcommand\detectTypeAndHighlight@prolog
{%
  % First, assume that we have an atom.
  \def\lst@thestyle{\PrologAtomStyle}%
  % Test whether we have a predicate and modify the style accordingly.
  \ifpredicate@prolog@%
    \def\lst@thestyle{\PrologPredicateStyle}%
  \else
    % Test whether we have a predicate and modify the style accordingly.
    \expandafter\splitfirstchar@prolog\expandafter{\the\lst@token}%
    % Check whether the identifier starts by an underscore.
    \expandafter\ifx\@testChar@prolog\underscore@prolog%
      % Check whether the identifier is '_' (anonymous variable)
      \ifnum\lst@length=1%
        \let\lst@thestyle\PrologAnonymVarStyle%
      \else
        \let\lst@thestyle\PrologVarStyle%
      \fi
    \else
      % Check whether the identifier starts by a capital letter.
      \currentchar@prolog=65
      \loop
        \expandafter\ifnum\expandafter`\@testChar@prolog=\currentchar@prolog%
          \let\lst@thestyle\PrologVarStyle%
          \let\iterate\relax
        \fi
        \advance \currentchar@prolog by 1
        \unless\ifnum\currentchar@prolog>90
      \repeat
    \fi
  \fi
}
\newcommand\splitfirstchar@prolog{}
\def\splitfirstchar@prolog#1{\@splitfirstchar@prolog#1\relax}
\newcommand\@splitfirstchar@prolog{}
\def\@splitfirstchar@prolog#1#2\relax{\def\@testChar@prolog{#1}}

% helper macro for () delimiters
\def\beginlstdelim#1#2%
{%
  \def\endlstdelim{\PrologOtherStyle #2\egroup}%
  {\PrologOtherStyle #1}%
  \global\predicate@prolog@false%
  \withinparens@prolog@true%
  \bgroup\aftergroup\endlstdelim%
}

% language name
\newcommand\lang@prolog{Prolog-pretty}
% ``normalised'' language name
\expandafter\lst@NormedDef\expandafter\normlang@prolog%
  \expandafter{\lang@prolog}

% language definition
\expandafter\expandafter\expandafter\lstdefinelanguage\expandafter%
{\lang@prolog}
{%
  language            = Prolog,
  keywords            = {},      % reset all preset keywords
  showstringspaces    = false,
  alsoletter          = (,
  alsoother           = @$,
  moredelim           = **[is][\beginlstdelim{(}{)}]{(}{)},
  MoreSelectCharTable =
    \lst@DefSaveDef{`(}\opparen@prolog{\global\predicate@prolog@true\opparen@prolog},
}

% Hooking into listings to test each ``identifier''
\newcommand\@ddedToOutput@prolog\relax
\lst@AddToHook{Output}{\@ddedToOutput@prolog}

\lst@AddToHook{PreInit}
{%
  \ifx\lst@language\normlang@prolog%
    \let\@ddedToOutput@prolog\@testChar@prolog%
  \fi
}

\lst@AddToHook{DeInit}{\renewcommand\@ddedToOutput@prolog{}}

\makeatother
%
% --- end of ugly internals ---


% --- definition of a custom style similar to that of Pygments ---
% custom colors
\definecolor{PrologPredicate}{RGB}{000,031,255}
\definecolor{PrologVar}      {RGB}{024,021,125}
\definecolor{PrologAnonymVar}{RGB}{000,127,000}
\definecolor{PrologAtom}     {RGB}{186,032,032}
\definecolor{PrologComment}  {RGB}{063,128,127}
\definecolor{PrologOther}    {RGB}{000,000,000}

% redefinition of user macros for Prolog style
\renewcommand\PrologPredicateStyle{\color{PrologPredicate}}
\renewcommand\PrologVarStyle{\color{PrologVar}}
\renewcommand\PrologAnonymVarStyle{\color{PrologAnonymVar}}
\renewcommand\PrologAtomStyle{\color{PrologAtom}}
\renewcommand\PrologCommentStyle{\itshape\color{PrologComment}}
\renewcommand\PrologOtherStyle{\color{PrologOther}}

% custom style definition 
\lstdefinestyle{Prolog-pygsty}
{
  language     = Prolog-pretty,
  upquote      = true,
  stringstyle  = \PrologAtomStyle,
  commentstyle = \PrologCommentStyle,
  literate     =
    {:-}{{\PrologOtherStyle :-}}2
    {,}{{\PrologOtherStyle ,}}1
    {.}{{\PrologOtherStyle .}}1
}

% global settings
\lstset
{
  captionpos = below,
  frame      = single,
  columns    = fullflexible,
  basicstyle = \ttfamily,
}

\lstnewenvironment{code}
    {\lstset{}%
      \csname lst@SetFirstLabel\endcsname}
    {\csname lst@SaveFirstLabel\endcsname}
    \lstset{
       style      = Prolog-pygsty    
    }

